Don't sit on the fence: A static analysis approach to automatic fence insertion

Modern architectures rely on memory fences to prevent undesired weakenings of memory consistency. As the fences' semantics may be subtle, the automation of their placement is highly desirable. But precise methods for restoring consistency do not scale to deployed systems code. We choose to trade some precision for genuine scalability: our technique is suitable for large code bases. We implement it in our new musketeer tool, and detail experiments on more than 350 executables of packages found in Debian Linux 7.1, e.g. memcached (about 10000 LoC).

==> Makefile <==
FILE=main
DVIPS=dvips
LATEX=rubber
XDVI=xdvi  -s 7 -paper a4 -expert
EDITOR=emacs
GV=gv
LPR=lpr
HEVEA=hevea
HEVEAOPTS=-fix
HACHA=hacha
HACHAOPTS=-tocbis
FIG=

DEPENDS=main.tex macros.tex litmus.tex abstract.tex introduction.tex related-work.tex \
motivation.tex cycles.tex detection.tex inference.tex \
comparison.tex conclusion.tex insertion.tex main.tex $(FIG)

all: ps pdf

$(FILE).dvi: $(DEPENDS)

default: $(FILE).dvi
fig: $(FIG)

ps: $(FILE).ps

pdf: $(FILE).ps
	ps2pdf $(FILE).ps

broch: $(FILE).2.ps

gv: $(FILE).ps
	$(GV) $(FILE).ps&

lpr: $(FILE).ps
	$(LPR) $(FILE).ps

bib: $(FILE).dvi
	$(LATEX) $(FILE).tex
	bibtex $(FILE)
	$(LATEX) $(FILE).tex

force:
	$(LATEX) $(FILE).tex

index.html: $(FILE).html
	$(HACHA) $(HACHAOPTS) $(FILE).html

$(FILE).html: $(DEPENDS) sig-alt-full.hva
	$(HEVEA) $(HEVEAOPTS) $(FILE)

view:
	evince main.pdf &

clean:
	/bin/rm -f *.aux *.dvi *.log *.dep *.bbl *.blg $(FILE).pdf $(FILE).ps
	/bin/rm -f log
	/bin/rm -f *.advi
	/bin/rm -f *.pstex *.pstex_t *.png

%.dvi: %.tex
	$(LATEX) $*.tex || /bin/rm -f $*.dvi

%.advi: %.dvi
	dvicopy $< $@

%.ps: %.dvi
	$(DVIPS) -o $*.ps $*.dvi

%.2.ps: %.ps
	brochure $*.ps

%.png: %.dot
	sh mkpng.sh $* dot > $* .png && qiv $*.png && /bin/rm -f $*.png 

